Depletion and fractionation of nitrogen in collapsing cores

Measurements of the nitrogen isotopic ratio in Solar System comets show a constant value, ~140, which is three times lower than the protosolar ratio, a highly significant difference that remains unexplained. Observations of static starless cores at early stages of collapse confirm the theoretical expectation that nitrogen fractionation in interstellar conditions is marginal for most species. Yet, observed isotopic ratios in N2H+ are at variance with model predictions. These gaps in our understanding of how the isotopic reservoirs of nitrogen evolve, from interstellar clouds to comets, and, more generally, to protosolar nebulae, may have their origin in missing processes or misconceptions in the chemistry of interstellar nitrogen. So far, theoretical studies of nitrogen fractionation in starless cores have addressed the quasi-static phase of their evolution such that the effect of dynamical collapse on the isotopic ratio is not known. In this paper, we investigate the fractionation of 14N and 15N during the gravitational collapse of a pre-stellar core through gas-phase and grain adsorption and desorption reactions. The initial chemical conditions, which are obtained in steady state after typically a few Myr, show low degrees of fractionation in the gas phase, in agreement with earlier studies. However, during collapse, the differential rate of adsorption of 14N- and 15N-containing species onto grains results in enhanced 15N:14N ratios, in better agreement with the observations. Furthermore, we find differences in the behavior, with increasing density, of the isotopic ratio in different species. We find that the collapse must take place on approximately one free-fall timescale, based on the CO abundance profile in L183 [see the end in the PDF file]

==> general.tex <==
%
% Editing
%

\def \red#1{\textcolor{red}{#1}}
\def \blue#1{\textcolor{blue}{#1}}
\def \vert#1{\textcolor{green}{#1}}
\def \jaune{\textcolor{yellow}}
\def \magenta#1{\textcolor{magenta}{#1}}
\def \cyn#1{\textcolor{cyan}{#1}}
\def \etc{{\it etc}}
\def \ie{{\it i.e.}}
\def \eg{{\it e.g.}}
\def \via{{\it via}}
\def \idem{{\it idem}}
\def \infine{{\it in fine}}
\def \apost{{\it a posteriori}}
\def \afort{{\it a fortiori}}
\def \vs{{\it vs}}
\def \etal{{\it et al}}
\def \cad{c'est-\`a-dire}
\newcommand{\permil}{%
  \relax\ifmmode\promillezeichen
        \else\leavevmode\(\mathsurround=0pt\promillezeichen\)\fi}
\newcommand{\perth}{\textperthousand}
\newcommand\mydate{}
\edef\mydate{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
%
%-----------------------------------------------
% Mathematics
%\DeclareMathOperator{\sinc}{sinc}
\newcommand\sinc{{\rm sinc}}
\def \dix#1{\ensuremath{{\,\rm 10^{#1}}}}
\def \tdix#1{\ensuremath{{\,\times 10^{#1}}}}
\def \dth{\ensuremath{\ud\theta}}
\def \dph{\ensuremath{\ud\phi}}
\def \om{\ensuremath{{\Omega}}}
\def \dom{\ensuremath{\ud\om}}
\def \ohalf{\ensuremath{\Omega_{2\pi}}}
\def \ud   {\ensuremath{\,\mathrm{d}}}
\def \uD   {\ensuremath{\,\mathrm{D}}}
\def \udp  {\ensuremath{\partial}}
\def \dt#1{\ensuremath{\frac{d{#1}}{dt}}}
\def \dx#1{\ensuremath{\frac{d{#1}}{dx}}}
\def \dtot#1#2{\ensuremath{\frac{d{#1}}{d{#2}}}}
\def \dpdt#1{\ensuremath{\frac{\partial{#1}}{\partial{t}}}}
\newcommand\dlog[1]{\ensuremath{\frac{d#1}#1}}
\newcommand\dpdr[1]{\ensuremath{\frac{\partial{#1}}{\partial{r}}}}
\newcommand\dpartij[3]{\ensuremath{\partial^{#2}_{#1}#3}}
\newcommand\dpart[2]{\ensuremath{\partial_{#1}#2}}
\newcommand\fdpart[2]{\ensuremath{\frac{\partial{#1}}{\partial{#2}}}}
\newcommand \fracp[2]{\ensuremath{\left(\frac{#1}{#2}\right)}}
\newcommand \fracc[2]{\ensuremath{\left[\frac{#1}{#2}\right]}}
\def \nbb{\ensuremath{{\rm I\!N}}} % ensemble des entiers
\def \rbb{\ensuremath{{\rm I\!R}}} % ensemble des reels
\def \dint {\displaystyle\int}
\def \dsum {\displaystyle\sum}
\def \lp   {\ensuremath{\left(}}
\def \rp   {\ensuremath{\right)}}
\def \lc   {\ensuremath{\left[}}
\def \rc   {\ensuremath{\right]}}
\def \lb   {\ensuremath{\left\{}}
\def \rb   {\ensuremath{\right\}}}
\newcommand\pfr[2]{\ensuremath{\lp\frac{#1}{#2}\rp}}
\newcommand\cfr[2]{\ensuremath{\lc\frac{#1}{#2}\rc}}
\newcommand\bfr[2]{\ensuremath{\lb\frac{#1}{#2}\rb}}
\def \aver#1{\ensuremath{\langle #1 \rangle}}
\def \<{\ensuremath{\langle}}
\def \>{\ensuremath{\rangle}}
\def \lr{\ensuremath{\leftrightarrow}}
\def \lra{\ensuremath{\longrightarrow}}
\def \ra{\ensuremath{\rightarrow}}
\def \la{\ensuremath{\leftarrow}}
\def \Ra{\ensuremath{\Rightarrow}}
\def \LRa{\ensuremath{\Leftrightarrow}}
\def \vdot#1#2{\ensuremath{\vect{{#1}}\cdot\vect{{#2}}}}
\def \vcro#1#2{\ensuremath{\vect{{#1}}\times\vect{{#2}}}}
\def \rot{\ensuremath{\vect{\nabla}\times}}
\def \div#1{\ensuremath{\vect{\nabla}\cdot{#1}}}
\def \grad#1{\ensuremath{\vect{\nabla}(#1)}}
\def \lapla{\ensuremath{\nabla^2}}
\def \scal#1#2{\ensuremath{\vec{#1}\cdot\vec{#2}}}
\newcommand \scalar[2]{\ensuremath{\vec{#1}\cdot\vec{#2}}}
\newcommand\logd{\ensuremath{\log_{10}}}
\newcommand\cplx[1]{\ensuremath{\underline{#1}}}
\newcommand\ccplx[1]{\ensuremath{\cplx{#1}^*}}
%
%
%
% ------------------------------------------------------------
%
% Physics and chemistry
%
\def \kb{\ensuremath{k_B}} % {\rm B}}}
\def \vth{\ensuremath{{v_{\rm th}}}}
\newcommand\bpos{\ensuremath{B_\perp}}
\newcommand\blos{\ensuremath{B_\parallel}}
%
%
% ------------------------------------------------------------
%
% General units
%
\def \hz{\ensuremath{{\rm Hz^{-1}}}}
\def \ang{\ensuremath{{\rm \mathring{A}}}}
\def \micr{\ensuremath{\mu {\rm m}}}
\def \pc{\ensuremath{{\rm pc}}}
\def \au{\ensuremath{{\rm au}}}
\def \ua{\ensuremath{{\rm ua}}}
\def \K{\ensuremath{{\rm K}}}
\def \per#1{\ensuremath{\,{\rm #1}^{-1}}}
\def \unit#1#2{\ensuremath{\,{\rm #1}^{#2}}}
\def \muG{\ensuremath{\mu {\rm G}}}
\def \mmm{\ensuremath{{\,\rm m^{-3}}}}
\def \mm{\ensuremath{{\,\rm m^{-2}}}}
\def \perm{\ensuremath{{\,\rm m^{-1}}}}
\def \percm{\ensuremath{{\,\rm cm^{-1}}}}
\def \cc{\ensuremath{{\,\rm cm^{-2}}}}
\def \ccc{\ensuremath{{\,\rm cm^{-3}}}}
\def \cccs{\ensuremath{~\rm cm^3\,s^{-1}}}
\def \gccc{\ensuremath{{\,\rm g\,cm^{-3}}}}
\def \cm{\ensuremath{{\,\rm cm}}}
\def \cmm{\ensuremath{{\,\rm cm^2}}}
\def \cmmm{\ensuremath{{\,\rm cm^3}}}
\def \ctwo{\ensuremath{{\,\rm cm^2}}}
\def \cthr{\ensuremath{{\,\rm cm^3}}}
\def \mtwo{\ensuremath{{\,\rm m^2}}}
\def \mthr{\ensuremath{{\,\rm m^3}}}
\def \pers{\ensuremath{{\,\rm s^{-1}}}}
\def \perm{\ensuremath{{\,\rm min^{-1}}}}
\def \perh{\ensuremath{{\,\rm hr^{-1}}}}
\def \peryr{\ensuremath{{\,\rm yr^{-1}}}}
\def \peran{\ensuremath{{\,\rm an^{-1}}}}
\def \yr{\ensuremath{{\,\rm yr}}}
\def \an{\ensuremath{{\,\rm an}}}
\def \cms{\ensuremath{{\,\rm cm\,s^{-1}}}}
\def \ms{\ensuremath{{\,\rm m\,s^{-1}}}}
\def \cmss{\ensuremath{{\,\rm cm\,s^{-2}}}}
\def \mss{\ensuremath{{\,\rm m\,s^{-2}}}}
\def \kms{\ensuremath{{\rm\,km\,s^{-1}}}}
\def \mstar{\ensuremath{M_\star}}
\def \rstar{\ensuremath{R_\star}}
\def \lstar{\ensuremath{L_\star}}
\def \rsol{\ensuremath{R_{\odot}}}
\def \lsol{\ensuremath{L_{\odot}}}
\def \msol{\ensuremath{{M_{\odot}}}}
\def \msolpc{\ensuremath{M_{\odot}\,{\rm pc}^{-1}}}
\def \cckms{\ensuremath{{\rm\,cm^{-2}\,(km/s)^{-1}}}}
\def \kmspc{\ensuremath{{\rm\,km\, s^{-1}\,pc^{-1}}}}
\def \cccK{\ensuremath{{\rm\,cm^{-3}\,\K^{-1}}}}
\def \kkms{\ensuremath{{\rm\,K\,km\,s^{-1}}}}
\def \cmcmg{\ensuremath{{\rm\,cm^2\,g^{-1}}}}
\newcommand{\ccg}{\ensuremath{\rm\,cm^2\,g^{-1}}}
\newcommand{\gcc}{\ensuremath{\rm\,g\,cm^{-2}}}
\def \mmkg{\ensuremath{{\rm\,m^2\,kg^{-1}}}}
\def \mkkms{\ensuremath{\rm\,mK\kms}}
\def \ster{\ensuremath{{\rm\,sr}^{-1}}}
%
% Astrophysics
\def \gam{\ensuremath{\gamma}-ray}
\def \vlsr{\ensuremath{v_{{\rm LSR}}}}
\def \arcmin{\ensuremath{^{\scriptscriptstyle\prime}}}
\def \arcsec{\ensuremath{^{\scriptscriptstyle\prime\prime}}}
\def \degr{\ensuremath{{^{\circ}}}}
\def \hms#1#2#3{\ensuremath{{\,\rm {#1}^h{#2}^m{#3}^s}}}
\def \dms#1#2#3{\ensuremath{{#1}^{\circ}{#2}\arcmin{#3}\arcsec}}
\def \lii{\ensuremath{\ell_{{\rm II}}}}
\def \bii{\ensuremath{b_{{\rm II}}}}
\def \Nh{\ensuremath{N_{{\rm H}}}}
\def \Nhi{\ensuremath{N_{{\rm HI}}}}
\def \Nhh{\ensuremath{N_{{\rm H_2}}}}
\def \av{\ensuremath{A_{{\rm V}}}}
\def \ak{\ensuremath{A_{{\rm K}}}}
\def \ebv{\ensuremath{E_{{\rm B-V}}}}
\def \nh{\ensuremath{n_{{\rm H}}}}
\def \nhh{\ensuremath{n_{{\ce{H2}}}}}
\def \mh{\ensuremath{m_{{\rm H}}}}
%
% Astrochemistry
%
\def \reac#1#2{\begin{equation}\label{eq:#1}\ce{#2}\end{equation}}
\def \reacnn#1{\[\ce{#1}\]}
\def \form#1{\ensuremath{\Phi(\ce{#1})}}
\def \dest#1{\ensuremath{\Delta(\ce{#1})}}
\def \tw   {\ensuremath{^{12}}}
\def \th   {\ensuremath{^{13}}}
\def \twc  {\ce{^{12}C}}
\def \thc  {\ce{^{13}C}}
\def \hep  {\ensuremath{{\rm He^+}}}
\def \hii  {\ensuremath{{\rm \textsc{HII}}}}
\def \hi   {\ensuremath{{\rm \textsc{HI}}}}
\def \hh   {\ensuremath{{\ce{H2}}}}
\def \h    {\ensuremath{{\rm H}}}
\def \hp   {\ensuremath{{\rm H^+}}}
\def \hhp  {\ensuremath{{\rm H_2^+}}}
\def \hhhp {\ensuremath{{\rm H_3^+}}}
\def \hho  {\ensuremath{{\rm H_2O}}}
\def \hcop {\ensuremath{{\rm HCO^+}}}
\def \hthcop {\ensuremath{{\rm H\thc O^+}}}
\def \co   {\ensuremath{{\rm CO}}}
\def \sixo   {\ensuremath{{\rm ^{16}O}}}
\def \eigo   {\ensuremath{{\rm ^{18}O}}}
\def \twCO {\ensuremath{{\rm ^{12}CO}}}
\def \thCO {\ensuremath{{\rm ^{13}CO}}}
\def \cdo  {\ensuremath {{\rm C^{18}O}}}
\def \cdso {\ensuremath {{\rm C^{17}O}}}
\def \thcdo{\ensuremath {{\rm ^{13}C^{18}O}}}
\def \thcp {\ensuremath {{\rm ^{13}C^+}}}
\def \cp   {\ensuremath {{\rm ^{12}C^+}}}
\def \chp  {\ensuremath {{\rm CH^+}}}
\def \cch  {\ensuremath {{\rm C_2H}}}
\def \cfp  {\ensuremath {{\rm CF^+}}}
\def \hf   {\ensuremath {{\rm HF}}}
\def \chhp {\ensuremath {{\rm CH_2^+}}}
\def \chhhp{\ensuremath {{\rm CH_3^+}}}
\def \htco {\ensuremath {{\rm H^{13}CO^{+} }}}
\def \dcop {\ensuremath {{\rm DCO^{+} }}}
% N bearing species
\def \nhhh {\ensuremath {{\rm NH_3}}}
\def \nnhp {\ensuremath {{\rm N_2H^{+}}}}
\def \nht  {\ensuremath {{\rm NH}_3}}
\def \nn   {\ensuremath {{\rm N_2 }}}
\def \cn   {\ensuremath {{\rm CN}}}
%\def \thcn {\ensuremath {{\rm ^{13}CN}}}
\def \thcn {\ce{^{13}CN}}
\def \foun {\ce{^{14}N}}
\def \fifn {\ce{^{15}N}}
\def \dens#1{\ensuremath{n(\ce{#1})}}
\def \ab#1{\ensuremath{[\ce{#1}]}}
%
%
% Fourier transform
\def \deftf#1{\ensuremath{{\cal F}[#1]}}
%\def \deftf#1{\ensuremath{{\rm FT}[#1]}}
\def \tf#1{\ensuremath{\widetilde{#1}}}
\def \tf#1{\ensuremath{\underline{#1}}}
\def \itf#1{\ensuremath{{\cal F}^{-1}#1}}
\def \xl{\ensuremath{x_\lambda}} % spatial frequency
\def \yl{\ensuremath{y_\lambda}} % spatial frequency
\def \ul{\ensuremath{u_\lambda}} % spatial frequency
\def \thl{\ensuremath{\theta_\lambda}} % reciprocal coordinate
%
% Quantum mechanics
%
\def \vect#1{\ensuremath{\vec{#1}}}
\def \op#1{\ensuremath{\hat{#1}}}
\def \ham{\ensuremath{{\cal H}}}
\def \wftot{\ensuremath{\Psi}}
\def \wfsp{\ensuremath{\phi}}
\def \wfspin{\ensuremath{\sigma}}
\def \wf{\ensuremath{\psi}}
\def \rmas{\ensuremath{\widetilde{m}}} % Reduced mass
\def \elec{\ensuremath{\rm e^-}}
%
% Angular momenta
%
\def \am{\ensuremath{\textsf{AM}}}
\def \oam{\ensuremath{\ell}}
\def \voam{\ensuremath{\vect{\ell}}}
\def \vl{\vect{l}}
\def \vs{\vect{s}}
\def \vj{\vect{j}}
\def \vi{\vect{i}}
\def \vf{\vect{f}}
\def \vli{\ensuremath{\vect{l}_i}}
\def \vsi{\ensuremath{\vect{s}_i}}
\def \vji{\ensuremath{\vect{j}_i}}
\def \vL{\vect{L}}
\def \vS{\vect{S}}
\def \vJ{\vect{J}}
\def \vI{\vect{I}}
\def \vF{\vect{F}}
\def \vr{\ensuremath{{\vect{r}}}}
\def \vR{\ensuremath{{\vect{R}}}}
%
\def \vbint{\ensuremath{\vec{B}_{\rm int}}}
\def \epot{\ensuremath{{\cal E}}}
\def \vso{\ensuremath{V_{\rm s-o}}}
%----------------------------------
%
% Radiation and photometry
%
% Units
\def \jy{\ensuremath{{\rm Jy}}}
\def \jysr{\ensuremath{{{\,\rm Jy\,sr^{-1}}}}}
\def \Mjysr{\ensuremath{{{\,\rm MJy\,sr^{-1}}}}}
\def \mjybeam{\ensuremath{{{\,\rm mJy/beam}}}}
\def \jkms{\ensuremath{{\,\jy\,\kms}}}
\def \lumsi{\ensuremath{{\,\rm W\,\mm}}}
\def \lumcgs{\ensuremath{{\,\rm erg\,\cc}}}
\def \fluxsi{\ensuremath{{\,\rm W\,\mm}}}
\def \intintsi{\ensuremath{{\,\rm W\,\mm\,sr^{-1}}}}
\def \intintcgs{\ensuremath{{\,\rm erg\pers\,\cm\,sr^{-1}}}}
\def \fluxcgs{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}}}}
\def \fdenscgs{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}\,Hz^{-1}}}}
\def \fdenssi{\ensuremath{{\,\rm W\,m^{-2}\,Hz^{-1}}}}
\def \ispecsi{\ensuremath{{\,\rm W\,m^{-2}\,Hz^{-1}\,sr^{-1}}}}
\def \ispecsiwl{\ensuremath{{\,\rm W\,m^{-2}\,m^{-1}\,sr^{-1}}}}
\def \ispec{\ensuremath{{\,\rm erg\,s^{-1}\,cm^{-2}\,Hz^{-1}\,sr^{-1}}}}
\def \emiss{\ensuremath{{\,\rm erg\, s^{-1}\, cm^{-3}}}}
\def \emisscoef{\ensuremath{{\,\rm erg\, s^{-1}\, cm^{-3}\,sr^{-1}\,Hz^{-1}}}}
\def \ergccc{\ensuremath{{\,\rm erg\, cm^{-3}}}}
\def \ergs{\ensuremath{{\,\rm erg\, s}}}
\def \jous{\ensuremath{{\,\rm J\, s}}}
%
\def \aul{\ensuremath{A_{ul}}}
\def \bul{\ensuremath{B_{ul}}}
\def \blu{\ensuremath{B_{lu}}}
\def \cul{\ensuremath{C_{ul}}}
\def \clu{\ensuremath{C_{lu}}}
\def \gul{\ensuremath{{\gamma_{ul}}}}
\def \glu{\ensuremath{{\gamma_{lu}}}}
\def \inu{\ensuremath{I_\nu}}
\def \ibg{\ensuremath{I_{\rm bg}}}
\def \jnu{\ensuremath{J_\nu}}
\def \anu{\ensuremath{{\alpha_\nu}}}
\def \knu{\ensuremath{{\kappa_\nu}}}
\def \snu{\ensuremath{{S_\nu}}}
\def \fnu{\ensuremath{{F_\nu}}}
\def \bnu{\ensuremath{B_\nu}}
\def \pnu{\ensuremath{p_\nu}}
\def \Pnu{\ensuremath{P_\nu}}
\def \efft{\ensuremath{\widetilde{T}}}
\def \etbr{\ensuremath{\widetilde{T}_{\rm B}}}
\def \etbg{\ensuremath{\widetilde{T}_{\rm bg}}}
\def \etex{\ensuremath{\widetilde{T}_{\rm ex}}}
\def \etkin{\ensuremath{\widetilde{T}_{\rm kin}}}
\def \nc{\ensuremath{n_{\rm crit}}}
\def \d{{\ud}}
\def \sr{\ensuremath{{\rm sr^{-1}}}}
\def \jbar{\ensuremath{\overline{J}}}
\def \udot#1{\ensuremath{\dot{#1}}}
\def \mbol{\ensuremath{m_{\rm bol}}}
\def \Mbol{\ensuremath{M_{\rm bol}}}
\def \lbol{\ensuremath{L_{\rm bol}}}
\def \teff{\ensuremath{T_{\rm eff}}}
%-----------------------------------------------
%
% Radio astronomy
%
%
\newcommand \tante{\ensuremath{T_{\rm A}}}
\newcommand \tant{\ensuremath{T_{{\rm A}}^\star}}
\newcommand \tantc{\ensuremath{T_{\rm A,c}^*}}
\newcommand \tmb{\ensuremath{{T_{{\rm mb}}}}}
\newcommand \tmbc{\ensuremath{T_{{\rm mb,c}}}}
\newcommand \feff{\ensuremath{F_{{\rm{eff}}}}}
\newcommand \beff{\ensuremath{B_{{\rm{eff}}}}}

\def \off{{\tt OFF}}
\def \terr{\ensuremath{T_{\rm err}}}
% \def \tA{\ensuremath{T_{\rm A}}}
% \def \tB{\ensuremath{T_{\rm B}}}
% \def \tR{\ensuremath{T_{\rm R}}}
\newcommand \mb{\ensuremath{{\om_{\rm mb}}}}
\newcommand \sou{\ensuremath{{\om_{\rm S}}}}
\newcommand \tbr{\ensuremath{T_{{\rm B}}}}
\newcommand \tkin{\ensuremath{T_{{\rm kin}}}}
\newcommand \texc{\ensuremath{T_{{\rm ex}}}}
\newcommand \tgas{\ensuremath{T_{{\rm gas}}}}
\newcommand \tdust{\ensuremath{T_{\rm dust}}}
\newcommand \tbg{\ensuremath{T_{{\rm bg}}}}
\newcommand \aper{\ensuremath{{\cal A}}}  % Complexe aperture function
\newcommand \ffield{\ensuremath{f}}       % Far-field pattern
\newcommand \pp{\ensuremath{{\cal P}}}    % Far-field power pattern
\newcommand \ppnu{\ensuremath{{\cal P}_\nu}}    % Far-field power pattern
\newcommand \otf{\ensuremath{{\cal T}}}   % Telescope transfer function
\newcommand \eant{\ensuremath{E_{\rm aper}}}
\newcommand \efar{\ensuremath{E_{\rm ff}}}
\newcommand \pbeam{\ensuremath{{\cal P}(\Omega)}}
\newcommand \pmbeam{\ensuremath{{\cal P}_0(\Omega)}}
\newcommand \perr{\ensuremath{{\cal P}_e(\Omega)}}
\newcommand \perrk{\ensuremath{{\cal P}_{e,k}(\Omega)}}
\newcommand \pwall{\ensuremath{{\cal P}_{4\pi}}}
\newcommand \pwhalf{\ensuremath{{\cal P}_{2\pi}}}
\newcommand \pwmb{\ensuremath{{\cal P}_{\rm mb}}}
\newcommand \pwsou{\ensuremath{{\cal P}_S}}
\newcommand \tsou{\ensuremath{T_{\rm sou}}}
\newcommand \tgr{\ensuremath{T_{\rm gr}}}
\newcommand \tcal{\ensuremath{T_{{\rm cal}}}}
\newcommand \tsys{\ensuremath{T_{\rm sys}}}
\newcommand \tsky{\ensuremath{T_{\rm sky}}}
\newcommand \trec{\ensuremath{T_{\rm rec}}}
\newcommand \temi{\ensuremath{T_{\rm sky}}}
\newcommand \tspil{\ensuremath{T_{\rm spillover}}}
\newcommand \tatm{\ensuremath{T_{\rm atm}}}
\newcommand \thot{\ensuremath{T_{\rm hot}}}
\newcommand \tcol{\ensuremath{T_{\rm col}}}
\newcommand \etau{\ensuremath{e^{-\tau_\nu}}}
\newcommand \csou{\ensuremath{C_{\rm sou}}}
\newcommand \catm{\ensuremath{C_{\rm atm}}}
\newcommand \chot{\ensuremath{C_{\rm hot}}}
\newcommand \ccol{\ensuremath{C_{\rm col}}}
\newcommand \nulo{\ensuremath{\nu_{\rm LO}}}
\newcommand \nusky{\ensuremath{\nu_{\rm sky}}}
\newcommand \nuif{\ensuremath{\nu_{\rm IF}}}
\newcommand \philo{\ensuremath{\Phi_{\rm LO}}}
\newcommand \phisky{\ensuremath{\Phi_{\rm sky}}}
%
% Interferometry
\def \vis{\ensuremath{{\cal V}}}
%
%
%----------------------------------
% Editing
\def \xe{\ensuremath{x_e}}
\def \Left{\textit{Left}}
\def \Right{\textit{Right}}
\def \mc#1#2{\multicolumn{#1}{c}{#2}}
\def \hlign#1#2{\noindent\centerline{\rule{#1\textwidth}{#2pt}\goodbreak}}
\def \fullw{1.0\hsize}
\def \fullh{0.85\textheight}
\def \fulh{0.75\textheight}
\def \mcite#1{{\centerline{\tiny\cite{#1}}}}
%\def \subtitle#1{\par{\centerline{\tiny #1}}}
\def \note#1{{\scriptsize #1}}
\def \fnote#1{{\par\noindent\tiny #1}}
\def \Htitle#1{\centerline{\Large \textbf{#1}}\hlign{1}{2}\bigskip}
\newcommand\entry[1]{\noindent\textbf{#1}}
\newcommand{\tabnote}{\footnotesize\flushleft \hspace{2em}\textsc{Note.}---}
\newcommand{\tabnotes}{\footnotesize\flushleft \hspace{2em}\textsc{Notes.}---}
\newcommand{\tabref}{\footnotesize\flushleft \hspace{2em}\textsc{References.}---}

\newcommand\htitle[1]{%
  \begin{center}
    \begin{minipage}[c]{0.8\hsize}
      \centering
      \Large
      \textbf{#1}
    \end{minipage}
  \end{center}\hlign{1}{1}\tableofcontents\hlign{1}{1}}

\newcommand \idx[1]{#1\index{#1}}
\newcommand \iidx[2]{#2\index{#1!#2}}
\newcommand \iiidx[2]{#1 #2\index{#1!#2}}
%\newcommand \refeq[1]{Eq.~(\ref{eq:[1]})}
\newcommand \req[1]{Eq.~(\ref{eq:#1})}
\newcommand \reqs[2]{Eqs.~(\ref{eq:#1})--(\ref{eq:#2})}
%\newcommand \rsec[1]{$\S$\ref{sec:#1}}
\newcommand \rsec[1]{Sect.~\ref{sec:#1}}
\newcommand \rapp[1]{Appendix~\ref{app:#1}}
\newcommand \rtab[1]{Table~\ref{tab:#1}}
\newcommand \rtabs[2]{Tables~\ref{tab:#1}--\ref{tab:#2}}
\newcommand \rfig[1]{Fig.~\ref{fig:#1}}
\newcommand \rfigs[2]{Figs.~\ref{fig:#1}--\ref{fig:#2}}
\newcommand \lfig[1]{\label{fig:#1}}
\newcommand \ltab[1]{\label{tab:#1}}
\newcommand\cits[1]{Sec.~\ref{sec:#1}}
\newcommand\labs[1]{\label{sec:#1}}


==> journal_short.tex <==
\def \aal{A\&A Letters}
\def \aap{A\&A}
\def \aaps{A\&AS}
\def \aapr{Astron. Astrophys. Rev.}
\def \apss{Astroph. \& Sp. Sc.}
\def \aj{AJ}
\def \apj{ApJ}
\def \apjl{ApJL}
\def \apjs{ApJS}
\def \apl{Astrop. Lett.}
\def \araa{ARA\&A}
\def \bain{Bull. Astr. Inst. Netherlands}
\def \chemrev{Chemical Reviews}
%\def \gca{Geochim. Cosmochim. Ac.}
\def \gca{GCA}
\def \icarus{Icarus}
\def \inprep{\textit{in prep.}}
\def \jfm{JFM}
\def \mnras{MNRAS}
\def \nat{Nature}
\def \pasj{PASJ}
\def \pasp{PASP}
\def \pccp{Phys. Chem. Chem. Phys.}
\def \ppvi{Protostars \& Planets VI}
\def \prl{PRL}
\def \pra{Phys Rev A}
\def \prb{Phys Rev B}
\def \prc{Phys Rev C}
\def \prd{Phys Rev D}
\def \pre{Phys Rev E}
\def \qjras{Q. Jl R. astr. Soc.}
\def \rmp{Rev. Mod. Phy.}
\def \phypla{Phys. Plasmas}
\def \phyflu{Phys. Fluids}
\def \jphysb{Jour. of Physics B}
\def \pieee{Proc. IEEE}
\def \fcp{Fundamental Cosmic Physics}
\def \actaa{Acta Astronomica}
\def \ssr{Space Sci Rev}
\def \sci{Science}
\def \sub{submitted}
\def \epsl{E\&PS Letters}
\def \euphysb{Eur. Phys. J. B.}
\def \jcp{JCP}
\def \jpca{JPCA}
\def \mps{Meteor. \& Plan. Sc.}
\def \pnas{PNAS}
\def \jms{Jour. Molec. Spec.}
\def \pccp{PCCP}
\def \arfm{AR Flu Mech}
\def \molphys{Mol. Phys.}


==> latexfigs.tex <==
% Lenghts

\def\fullw{0.95\hsize}
\def\fullh{0.85\textheight}
\def\fulh{0.7\textheight}
% 
% Environments for figures
%
\def\land#1#2{\includegraphics[width=#1\hsize]{#2}}
\newcommand\port[2]{{\includegraphics[height=#1\textheight]{#2}}}
\newcommand\onefig[2]{\includegraphics[#1]{#2}}
\newcommand\hfig[2]{\includegraphics[width=#1\textwidth]{{#2}}}
\newcommand\vfig[2]{\includegraphics[height=#1\textheight]{{#2}}}
\newcommand\rotfig[3]{\includegraphics[angle=#1,width=#2\textheight]{#3}}
\newcommand\onehfig{\hfig}
\newcommand\onevfig{\vfig}

